Modern topics in relativistic spin dynamics and magnetism

Magnetism is a rich subject touching all aspects of physics. My goal with this dissertation is to explore spin and magnetic moments in \emph{relativistic} mechanics from both a quantum and classical perspective. We emphasize the special case of gyromagnetic ratio $g\!=\!2$ and its relationship to the algebraic spin structure of wave equations. In relativistic quantum mechanics, we investigate generalizations of the Dirac equation for arbitrary magnetic moments for fermions. We analyze the homogeneous magnetic field case and the Coulomb problem for hydrogen-like atoms with emphasis on the role of the anomalous magnetic moment (AMM). We explore alternative approaches which combine mass and the magnetic moment. Classically, we propose a relativistic covariant model of the Stern-Gerlach force via the introduction of a magnetic four-potential. This model modifies the covariant torque equations and unites the Amp\`erian and Gilbertian models for magnetic moments. We further study (transition) magnetic dipoles in Majorana neutrinos specifically analyzing the relationship between flavor mixing and electromagnetic (EM) fields. We demonstrate EM flavor mixing explicitly in the 2-flavor model and develop a dynamical mass basis with an EM rotation matrix. EM induced neutrino mass splitting is compared to neutrino mass hierarchy. An interesting application of these theoretical developments is to study primordial magnetization in the early universe during the hot dense electron-positron plasma epoch. We propose a model of magnetic thermal matter-antimatter plasmas. We analyze the paramagnetic characteristics of electron-positron plasma when exposed to an external primordial field. Future research outlooks include: Second order equations for anomalous quantum chromodynamic (QCD) moments, neutrino CP violation in strong EM fields, and fifth-dimension spin dynamics in Kaluza-Klein theory.

==> subtex/abstract.tex <==
%auto-ignore

%This is where the body of your abstract goes, limited to 150 words
%for a thesis, and 350 words for a dissertation or document.  The
%word count limits apply to the regular Abstract in the thesis and
%to the separate Special Abstract.  Use the same text for both; just
%adjust the margins and heading.  The abstract should summarize your
%work.  The UMI booklet listed in the resources section of the U of
%A manual provides some writing tips.  The abstract for a dissertation
%or document may be longer than one page; word count is more important
%than page length in this section.

%If you are doing a paper submission, submit one copy of the special 
%abstract, and two extra copies of your title page, in the box with 
%the final copies of your thesis.  If you are doing an electronic
%submission, you can ignore the special abstract.

Magnetism is a rich subject touching all aspects of physics. My goal with this dissertation is to explore spin and magnetic moments in \emph{relativistic} mechanics from both a quantum and classical perspective. We emphasize the special case of gyromagnetic ratio $g\!=\!2$ and its relationship to the algebraic spin structure of wave equations.

In relativistic quantum mechanics, we investigate generalizations of the Dirac equation for arbitrary magnetic moments for fermions. We analyze the homogeneous magnetic field case and the Coulomb problem for hydrogen-like atoms with emphasis on the role of the anomalous magnetic moment (AMM). We explore alternative approaches which combine mass and the magnetic moment. Classically, we propose a relativistic covariant model of the Stern-Gerlach force via the introduction of a magnetic four-potential. This model modifies the covariant torque equations and unites the Amp{\`e}rian and Gilbertian models for magnetic moments.

We further study (transition) magnetic dipoles in Majorana neutrinos specifically analyzing the relationship between flavor mixing and electromagnetic (EM) fields. We demonstrate EM flavor mixing explicitly in the 2-flavor model and develop a dynamical mass basis with an EM rotation matrix. EM induced neutrino mass splitting is compared to neutrino mass hierarchy.

An interesting application of these theoretical developments is to study primordial magnetization in the early universe during the hot dense electron-positron plasma epoch. We propose a model of magnetic thermal matter-antimatter plasmas. We analyze the paramagnetic characteristics of electron-positron plasma when exposed to an external primordial field. We determine the magnitude of a small polarization asymmetry is sufficient to generate field strengths in agreement with those measured today in deep intergalactic space.

Future research outlooks include: Second order equations for anomalous quantum chromodynamic (QCD) moments, neutrino CP violation in strong EM fields, and fifth-dimension spin dynamics in Kaluza-Klein theory.


==> subtex/acknowledgements.tex <==
%auto-ignore

%add acknowledgements here

In my long journey to obtain my PhD, I have benefited from the immense support and friendship of many people in my life. To them I am incredibly grateful.

I first would like to thank Professor Johann Rafelski who as my PhD advisor guided me on my physics journey towards ever increasing heights of knowledge and understanding. Most importantly, I was imbued with a humble awareness of our ignorance towards much of the universe's inner workings. I dearly hope we continue to chip away at those mysteries together. I also would like to thank Victoria Grossack for hosting many students including myself at her and Dr. Rafelski's lovely home. I promise future gluten-free pies which I am now bound to by the publication of this dissertation.

To my fellow research collaborators and simultaneous dear friends, I thank for our wonderful time spent together (in alphabetical order): Stefan Evens, Martin Formanek, Christopher Grayson, Will Price, Cheng Tao Yang. Our group trip to Budapest, Hungary and Prague, Czech Republic this past summer is a memory I will cherish forever. Stefan, I appreciate your eternal enthusiasm and love of older architecture---I owe you a visit, hold me to it! Martin, I won't forget your generous hospitality and your words that ``physics \emph{is} magic.'' Chris, thank you for the kind help the evening before my presentation at PP2023. Thank you Hannah Isaac and Will for saving me from being lost forever within Frankfurt Central station. Cheng Tao, our work on cosmology together has reinvigorated me. I look forward to many more years and publications together.

I thank my closest friends who I've known over many years of fellowship (in alphabetical order): Michael Burrell, Jordan Cohen, Elizabeth Fitzpatrick, Kyle Fitzpatrick, Michael France, Jesse Griggs, Jose Gross, Pedro Gross, Kevin Huffman, Alyssa Playford, and Sagar Samtani. To those in this group who I ride motorcycles with, it's with you I've known true freedom.

I lastly, though equally, thank my family who have supported and been there for me: My mom Maria Steinmetz, my cousins Cindy and Frank Ramos, my aunt and uncle Danuta and Bill Kemp.

Good health and long life to all.

==> subtex/dedication.tex <==
%auto-ignore

{
\itshape
I dedicate this dissertation to my dad, Christopher Steinmetz, who never really got to know me. I still got your copy of Kip Thorne's ``Black Holes \& Time Warps'' with the dust cover bookmarking page 172: The Equivalence of Mass and Energy. I think we would have gotten along swimmingly.
}

\vfill

{
\noindent Upon his dear friend Michele Besso's passing, Albert Einstein wrote a letter to Besso's family which ended with:
\centering\itshape
``Now he has departed from this strange world a little ahead of me. That means nothing. People like us, who believe in physics, know that the distinction between past, present, and future is only a stubbornly persistent illusion.''
}

\vfill

{
\centering\emph{
    The past, the now, the yet to come,\\
    All the same mechanical sum.\\
    Write down the rules, the laws we borrow,\\
    A glimpse of nature for all tomorrows.\\
}
---A meter of physics\,\\
}


